NeuroLogic A*esque Decoding: Constrained Text Generation with Lookahead Heuristics

The dominant paradigm for neural text generation is left-to-right decoding from autoregressive language models. Constrained or controllable generation under complex lexical constraints, however, requires foresight to plan ahead feasible future paths. Drawing inspiration from the A* search algorithm, we propose NeuroLogic A*esque, a decoding algorithm that incorporates heuristic estimates of future cost. We develop efficient lookahead heuristics that are efficient for large-scale language models, making our method a drop-in replacement for common techniques such as beam search and top-k sampling. To enable constrained generation, we build on NeuroLogic decoding (Lu et al., 2021), combining its flexibility in incorporating logical constraints with A*esque estimates of future constraint satisfaction. Our approach outperforms competitive baselines on five generation tasks, and achieves new state-of-the-art performance on table-to-text generation, constrained machine translation, and keyword-constrained generation. The improvements are particularly notable on tasks that require complex constraint satisfaction or in few-shot or zero-shot settings. NeuroLogic A*esque illustrates the power of decoding for improving and enabling new capabilities of large-scale language models.

==> fig/result_comGen_model.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{6pt}
\scriptsize
\setlength{\tabcolsep}{3.5pt}
    \centering
        \scalebox{1.09}{
    \begin{tabular}{ l|c c c c}
     \toprule
 \textbf{\hspace{1pt}Model} &   \textbf{BLEU-4}  & \textbf{METEOR}  &\textbf{CIDEr}   & \textbf{Coverage} \\ 
\midrule
 GPT-2 & 26.7 $ \rightarrow$ 28.2 &  30.2 $\rightarrow$ 30.8 & 14.7 $\rightarrow$ 15.2  &  97.7 $\rightarrow$ 97.8  \\
 UniLM & 31.5 $\rightarrow$ \textbf{32.0} & 31.7 $\rightarrow$ \textbf{31.9} & 16.6 $\rightarrow$ \textbf{16.7} & 97.8 $\rightarrow$ \underline{98.6} \\
 BART  & 30.6 $\rightarrow$ \underline{31.4} & 31.0 $\rightarrow$ \underline{31.4} & 15.9 $\rightarrow$ 16.2 & 98.7 $\rightarrow$ \textbf{98.7}\\
 T5  & 28.1 $\rightarrow$ 29.6 & 30.7 $\rightarrow$ 31.3 & 15.5 $\rightarrow$ \underline{16.4} & 98.5 $\rightarrow$ \underline{98.6} \\
    \bottomrule
    
    \end{tabular}}
    \caption{Experimental results in supervised on the C{\scriptsize OMMON}G{\scriptsize EN} test set. Under each column, $\alpha \rightarrow \beta$ shows the performance of \neurologic without ($\alpha$) and with ($\beta$) A$^\textbf{*}$ heuristics.
    \daniel{
    I think here the absolute scores are less important than the gap between them. 
    Concretely, compute the performance gaps and see if there is a pattern there. 
    }
    }  % 
    \label{tab:comGen_result_model}
\end{table}

==> section/1_intro_peter.tex <==




%%%%%%%%%%%%

Natural language generation has progressed in leaps and bounds in the recent past, largely driven by the left-to-right generation of causal language models like GPT-2 and GPT-3 \cite{radford2019language,Brown2020LanguageMA} \peter{cite more work}. While this has resulted in undeniable improvements, these models are prone to make locally probable decisions that result in text that is globally degenerate text \peter{cite}, or fails to incorporate constraints and control at the global level. (Figure~\ref{fig:teaser}). \peter{cite constrained papers}. 

The broader literature on artificial intelligence has considered this challenge thoroughly \peter{CITE}, with lookahead techniques such as A$^*$ search offering an effective solution to the local-decision/global-optimization mismatch. Inspired by this line, we propose A$^*$esque (stylized as A$^{\star}$), a heuristic method following the same logic, looking ahead to guide local decisions. 
\peter{Middle stuff}

\peter{Discussion of the limitations. }


Natural language generation has taken off thanks to large causal language models like GPT-2 and GPT-3. These follow a simple decoding paradigm--generate the next word given the \emph{past}, the generation so far--as in popular decoding algorithms such as sampling, truncated decoding, and beam search. Yet we often need to consider what \emph{future} a generated word will lead to as well

Progress in NLG has largely driven by causal language models like GPT-2 and GPT-3 \cite{radford2019language,Brown2020LanguageMA}, which generate sequentially, with decoding algorithms like greedy, sampling, beam search. While this paradigm generates the next word based on the past, already-generated text,  the effect it may have on future text--as such these methods are prone to making decisions that are probable based on past text, but result in degenerate text in the future, or fail to satisfy global constraints or controls. 

Rapid progress in natural language has been driven by sequential decoding with large causal language models like GPT-2 and GPT-3 \cite{radford2019language,Brown2020LanguageMA}. In this paradigm, the next word is predicted based on the past, already-generated text, yet considering past text alone is often insufficient--a probable next word may result in a globally degenerate generation \cite{holtzman2020curious,welleck2020neural} or one that fails to satisfy global constraints or controls \peter{CITE work on constrained/controllable gen} \lianhui{\cite{}. Indeed, generating high quality text requires considering the future, yet-to-be-generated text as well.

The broader literature on artificial intelligence has considered this challenge thoroughly \peter{CITE}, with lookahead techniques such as A$^*$ search offering an effective solution. Inspired by this line, we propose A$^*$esque (stylized as A$^{\star}$), a heuristic method following the same logic, looking ahead to guide local decisions towards globally optimal generations. 

==> section/2_method.tex <==

\subsection{Unconstrained generation.}

First we consider a standard decoding setting, 
$$\argmax_{\yb\in \mathcal{Y}} \log p_\theta(\yb|\xb).$$
We score candidates based on a combination of the history and estimated future, by using the likelihood of the lookahead as a heuristic.
That is, at the $t$'th step of decoding, we use \autoref{eqn:update4} with,
\begin{align}
    h(\yb_{\leq t+k}) &= \lambda \log p_\theta(\yb_{t+1:t+k}|\yb_{\leq t}, \xb),
\end{align}
where $\lambda$ controls how much we rely on the estimated future versus the history. 

\subsection{Constrained generation.}
% Lexically-constrained generation is the task of generating text subject to constraints on which tokens should or shouldn't appear.
For constrained generation, we extend \methodshort~\citep{lu-etal-2021-neurologic}-- a beam-based decoding algorithm that supports a wide class of logical constraints for lexically constrained generation-- with estimates of future contraint satisfaction.

\paragraph{Background: NeuroLogic.} 
\methodshort \citep{lu-etal-2021-neurologic} accepts lexical constraints in Conjunctive Normal Form (CNF):
\[\underbrace{\big(D_1 \lor D_2 \cdots \lor D_i \big)}_{C_1}\land \cdots \land \underbrace{\big(D_k \lor D_{k+1} \cdots \lor D_n \big)}_{C_L} \]
where each $D_j$ represents a single positive or negative constraint,  $D(\textbf{a}, \textbf{y})$ or $\neg D(\textbf{a}, \textbf{y})$, enforcing the phrase $\textbf{a}$ to be included in or omitted from \textbf{y}, respectively. \citeauthor{lu-etal-2021-neurologic} refer to each individual constraint $D_j$ as a \emph{literal}, and the disjunction of literals as a \emph{clause}, denoted as $C_i$. %\methodshort seeks optimal sequences in which all clauses are satisfied.

\methodshort is a beam-based approximate search for an objective which seeks fluent sequences in which all clauses are satisfied:
\vspace*{-3mm}
\begin{align*}
    \arg\max_{\textbf{y} \in \mathcal{Y}}p_\theta(\textbf{y}|\textbf{x}) - \lambda' \sum_{i=1}^{L} (1-C_i).
 \end{align*}
At each step of the search, \methodshort scores each of the $k\times |\mathcal{V}|$ candidates $(\yb_{<t},y_t)$ based on whether they (partially) satisfy new constraints,
\begin{align}
\label{eqn:neurologic-score}
    f(\yb_{\leq t}) = &\> \log p_\theta(\textbf{y}_{\leq t}|\xb) + \lambda_1 \max_{\substack{D(\textbf{a}_\textbf{i},\yb_{\leq t})}} \frac{|\hat{\textbf{a}}_\textbf{i}| }{|\textbf{a}_\textbf{i}|},
\end{align}
where the maximization is over a set of unsatisfied literals $\textbf{a}_i$ tracked by \methodshort,  and $\hat{\textbf{a}}_i$ is the prefix of $\textbf{a}_i$ in the ongoing generation.
For example, for $\yb_{\leq t}=$``\textit{The boy climbs an apple}'' and constraint $\textbf{a}_i$=`\textit{`apple tree}'', $\hat{\textbf{a}}_i$ is ``\textit{apple}''.
Intuitively, this function rewards candidates that are in the process of satisfying a multi-token constraint.

In lieu of taking the top-$k$ scoring candidates (\autoref{eqn:update4}), \methodshort prunes candidates that contain irreversibly unsatisfied clauses, groups the candidates to promote diversity, and selects high-scoring candidates from each group. 
We use the same pruning and grouping approach, and refer the reader to \citeauthor{lu-etal-2021-neurologic} for further details.
% At each time step, \methodshort chooses which candidates to expand next by 3 steps: \emph{pruning}, \emph{grouping}, and \emph{selecting} 

% We generalize \citep{lu-etal-2021-neurologic} by 

% \citet{lu-etal-2021-neurologic} propose NeuroLogic, which adjusts a candidate $(\yb_{<t},y_t)$'s scores based on whether the new token $y_t$ satisfies a logical constraint:
% \vspace*{-3mm}
% \begin{align*}
% \hat V = &\> \log p_\theta(y_t| \textbf{y}_{<t},\xb) + \lambda_1 \cdot \max_{\substack{D(\textbf{a}_\textbf{i}, \textbf{y}) \\ \in \> \textnormal{state S1}}} \frac{|\hat{\textbf{a}}_\textbf{i}| }{|\textbf{a}_\textbf{i}|}.
%  \end{align*}
% Here, \textcolor{red}{[TODO: concise explanation of the above. probably need to adjust the notation too (e.g. maybe we don't need state S1 here)]}. \ximing{Intuitively, this score function ranks candidates by log likelihood and gives a partial reward to the candidates in the process of satisfying a multi-tokens positive constraint.}
% \citet{lu-etal-2021-neurologic} show that using beam search with this scoring function empirically approximates,
% \vspace*{-3mm}
% \begin{align*}
%     \arg\max_{\yb \in \mathcal{Y}}P_\theta(\yb|\xb) - \lambda' \sum_{i=1}^{L} (1-C_i).
%  \end{align*}
% See the Appendix for a full review of NeuroLogic.

\paragraph{A*-NeuroLogic decoding.}
Our method improves upon the NeuroLogic scoring function with an estimate of future constraint satisfaction.
Our key addition is a lookahead heuristic that adjusts a candidate $(\yb_{<t},y_t)$'s score proportional to the probability of satisfying additional constraints in the lookahead $\yb_{t+1:t+k}$:
\begin{multline}
    h_{\text{future}}(\yb_{\leq t+k})= \\\lambda_2 \max_{D(\mathbf{a},\yb_{\leq t})} \log p_\theta(D(\mathbf{a},\yb_{t+1:t+k})|\xb,\yb_{\leq t}),
\end{multline}
where we define the probability that constraint $\mathbf{a}$ is satisfied using the most probable subsequence,
\begin{multline}
    p_\theta(D(\mathbf{a},\yb_{t+1:t+k})|\xb,\yb_{\leq t}) = \\
        \max_{i\in [1,k]} p_\theta(\yb_{t+i:t+i+|\mathbf{a}|}|\xb,\yb_{<t+i}),
\end{multline}
where $\lambda_2$ is a scaling hyperparameter.

Intuitively, this lookahead heuristic brings two benefits.
When $y_t$ is a token that would satisfy a multi-token constraint, the lookahead incorporates the score of the \textit{full} constraint. 
% \ximing{in this case, we also compute the later score in the following sentence, and take max over the two cases} \sean{can you clarify?}
When $y_t$ is a token that is not part of a constraint, the lookahead allows for incorporating the score of a future constraint that would be satisfied if $y_t$ was selected.

We add our lookahead heuristic to the \methodshort scoring function (\autoref{eqn:neurologic-score}), and call the resulting decoding procedure A$^*$-\methodshort.


\section{Method}
\ximing{Should we motivate the method session with constrained generation instead of talking unconstrained case first? The constrained generation is a NP hard problem, many constrained decoding algorithms are developed to approximate.... Inspired by the A* search in gaming/planning, we propose ... }
\daniel{
My personal taste: such high-level aspects about the motivation of the approach and where it works best should come much earlier (ideally, in the introduction). 
The paragraph here should mainly give a summary of how you are going to introduce the ideas  (the section organization).
}
\jungo{Agree with Daniel}

In this session, we present \method, which leverage estimated future state to guide current generation, in unconstrained and constrained generation, and demonstrate its use case on top of commonly used decoding methods in both settings.  (illustrated in figure \ref{fig:alg}, and detailed below).


\daniel{Nit suggestion: 
 (1) drop "unconstrained generation" header (makes the sectioning structure a bit complicated).
 (2) make "background"/"our approach" sections 
 (3) add a sentence in the earlier paragraph, along this line: "We introduce our algorithm for constrained algorithms, following by its application for the constrained decoding settings." }
 
\subsection{Unconstrained Generation}
\subsubsection{Background}
Given an input text $\textbf{x}$, the task of sequence-to-sequence generation is to generate a output text $\textbf{y}$ condition on input $\textbf{x}$. We assume that the model, parameterized by $\theta$, compute $P_\theta(\textbf{y}|\textbf{x})$ using the common left-to-right decomposition of the text probability,
\[P_\theta(\textbf{y}|\textbf{x}) = \prod_{t=1}^{n} P_\theta (\textbf{y}_t| \textbf{x}, \textbf{y}_{<t}).\]
\paragraph{Maximization-based decoding} Assuming that the model assigns higher probability to higher quality text, these decoding strategies search for the output text $\textbf{y}$ with the highest likelihood. Since exhaustive search for maximization is intractable, most common practice is to use beam search. 

\paragraph{Sampling-based decoding} Sampling has recently become a popular alternative decoding strategy to encourage diversity. Nucleus sampling~\cite{?} and top-k sampling~\cite{?} are the most commonly approaches, both of which sample from truncated Neural LM distributions, differing only in the strategy of where to truncate.

 \begin{figure*}[t]
\begin{center}
 \includegraphics[width=\linewidth]{fig/new_fig0.png}
 \includegraphics[width=\linewidth]{fig/fig1.pdf}
\end{center}
\caption{Illustration of decoding with \method for unconstrained and constrained generation. \probemoji $\:$ denotes token distribution $\tilde{P}_\theta(\textbf{y}_{t+i})$ and \embemoji $\:$ denotes fuzzy word embedding $\textbf{e}_{t+i}$. 
\daniel{Bottom figure, $P()$ should be $\tilde{P}(.)$ I think.}
}
\label{fig:alg}
\end{figure*}
\subsubsection{Our Approach: \method}
Common decoding strategies determine the probability of sampling from or choosing $w$ at time step $t$ purely based by sequence likelihood $P_\theta(\textbf{y}_{1:t} |\textbf{x},\textbf{y}_{t}\myeq w)$.  
However, several recent studies on seq2seq
generation have reported that sequence likelihood does not necessarily indicates high language quality.  \citep{holtzman-etal-2018-learning, fan-etal-2018-hierarchical}. 
\daniel{
I am not sure if I follow the logic here. 
Your lookahead algorithm is better than other ones (greedy, beam, etc) because it finds more probable solutions. 
This is  orthogonal (and somewhat contradictory to) Ari's argument (which was whether or not we should even search for **highest-probability** sequences.) 
}
\ximing{I agree. We're using looking ahead to estimate likelihood of future sequence or unstatisfied constraints . It's a bit contradictory to whether likelihood is a good measure. I think for unconstrained case, it's somewhat related to the findings in "if beam search is the answer, what's the question" where they found although beam search is thought to optimize for likelihood, there's this beam search blessing which enforces uniform information density, so that beam search returns better sequence than the high likelihood ones found in exact search.}
Thus,  \method propose to alternatively  score generation candidate based on \daniel{a combination of \sout{both}} the history and estimated future. 
\[P_\theta(\textbf{y}_{t}\myeq w |\textbf{x}, \textbf{y}_{<t} ) = 
\frac{P_\theta(\textbf{y}_{1:t} |\textbf{x},\textbf{y}_{t}\myeq w) \cdot \tilde{P}_\theta(\textbf{y}_{t+1:t+k} |\textbf{x},\textbf{y}_{1:t}, \textbf{y}_{t}\myeq w)^\lambda}{
\sum_{w\in V}
P_\theta(\textbf{y}_{1:t} |\textbf{x},\textbf{y}_{t}\myeq w) \cdot \tilde{P}_\theta(\textbf{y}_{t+1:t+k} |\textbf{x},\textbf{y}_{1:t}, \textbf{y}_{t}\myeq w)^\lambda
}\]
\daniel{
hmm .... this is a long equation :)  
Here is a modification  without numerator with $\propto$ indicating proportionality (which maybe needed to be clarified in a footnote). 
}
\jungo{there should be many ways to shrink this. x, for instance, can be suppressed.}
\begin{multline*}
P_\theta(\textbf{y}_{t}\myeq w |\textbf{x}, \textbf{y}_{<t} )  \propto P_\theta(\textbf{y}_{1:t} |\textbf{x},\textbf{y}_{t}\myeq w) \\ \times \tilde{P}_\theta(\textbf{y}_{t+1:t+k} |\textbf{x},\textbf{y}_{1:t}, \textbf{y}_{t}\myeq w)^\lambda,
\end{multline*}
where $\tilde{P}_\theta(\textbf{y}_{t+1:t+k} |\textbf{x},\textbf{y}_{1:t}, \textbf{y}_{t}\myeq w)$ is the estimated likelihood for future $k$ steps given candidate $w$ is chosen. 
\daniel{also say that $\textbf{y}_{t}\myeq w$ is folded inside $\textbf{y}_{1:t}$?}
$k$ is lookahead budget, controlling performance and runtime trade-off, and $\lambda$ is lookahead factor, controlling how much we rely on estimated future versus history. 


\daniel{Somewhere (here?) we need a sentence that says why computing  $\tilde{P}(.)$ can be non-trivial and requires proper estimation.}
To efficiently estimate  $\tilde{P}_\theta(\textbf{y}_{t+1:t+k} |\textbf{x},\textbf{y}_{1:t}, \textbf{y}_{t}\myeq w)$, we propose to fuzzily greedy decode $k$ more steps.
\daniel{
"Fuzzily" might raise eyebrows (note that "fuzzy" is a loaded term; cf. "fuzzy logic").  
How about a phrasings like these: "an semi-greedy" or "an approximate greedy"? 
}
A native version is to greedy decode $k$ more steps, however high dependency of LMs on local context makes such estimation highly affected by tokens decoded in the greedy steps and a less accurate reflection for the quality of candidate $w$. For fuzzy greedy decoding at $\textbf{y}_{t+i}$, we first compute the token distribution $\tilde{P}_\theta(\textbf{y}_{t+i})$ conditioned on the word embedding of its previous steps $\textbf{e}_{t+i-1}$: 

\begin{align*} 
\tilde{P}_\theta(\textbf{y}_{t+i}\myeq w |& \textbf{x}, \textbf{y}_{1:t+i-1} ) \\ 
& =\tilde{P}_\theta(\textbf{y}_{t+i}\myeq w |\textbf{x}, \textbf{e}_{1:t+i-1} ) \\ 
& = \frac{\exp(u_w/T)}{\sum_{w\in V} \exp(u_w/T)},
\end{align*}
where $u_w$ denotes the logit computed by LM for token $w$, and T denotes temperature, an adjustable parameter controlling how skew we want the token distribution to be. At the extreme case where $T\myeq0$, $\tilde{P}_\theta(\textbf{y}_{t+i})$ degrades to one-hot representation of greedily-decoded next token. 
Next, we compute the fuzzy word embedding $\textbf{e}_{t+i}$ for $\textbf{y}_{t+i}$ via
\[\textbf{e}_{t+i} = \tilde{P}_\theta(\textbf{y}_{t+i}|\textbf{x}, \textbf{y}_{1:t+i-1} ) \cdot \textbf{E},\]
where $\textbf{E}$ stands for word embedding table. The fuzzy word embedding $\textbf{e}_{t+i}$ is then fed into LM together with $\textbf{e}_{t+i-1}$ to estimate $\textbf{e}_{t+i+1}$. At the end, we compute likelihood in future $k$ step via \\ 
\[\tilde{P}_\theta(\textbf{y}_{t+1:t+k} |\textbf{x},\textbf{y}_{1:t}) = \prod_{i=1}^{k} \max_{w' \in V}\tilde{P}_\theta(\textbf{y}_{t+i}\myeq w' |\textbf{x}, \textbf{y}_{1:t+i-1} )\]
where the word representation of $\textbf{y}_{1:t+i-1}$ is obtained by concatenating the word embedding of $\textbf{y}_{1:t}$ and the fuzzy word embedding of $\textbf{y}_{t+1:t+i-1}$.

\daniel{Looks like we are using $\tilde{P}$ in two senses: here as a real-valued probability and earlier as a vector of probabilities over word distributions.}
\ximing{TODO: above is fuzzy decoding looking ahead, add beam and sampling looking ahead}


\subsection{Constrained Generation}
We generalize \textsc{A$^\textbf{*}$ Heuristic$\:$} to constrained generation as well. While \textsc{A$^\textbf{*}$ Heuristic$\:$} is compatible with any auto-regressive constrained decoding methods, such as method proposed by \cite{hokamp-liu-2017-lexically},\cite{post-vilar-2018-fast}, and \cite{hu-etal-2019-improved}, we demonstrate \method on top of \neurologic since \methodshort is the generalization of all previous auto-regressively constrained decoding methods and achieves the state-of-the-art performance. 

\subsubsection{Background: \neurologic}
\makeatletter
\newcommand{\stx}[1]{\mathpalette\giusti@stx{#1}}
\newcommand{\giusti@stx}[2]{%
  \mbox{%
    \medmuskip=\thinmuskip
    \thickmuskip=\thinmuskip
    $\m@th#1#2$%
  }%
}
\makeatother

\methodshort \citep{lu-etal-2021-neurologic} accepts lexical constraints in Conjunctive Normal Form (CNF):
\[\underbrace{\big(D_1 \lor D_2 \cdots \lor D_i \big)}_{C_1}\land \cdots \land \underbrace{\big(D_k \lor D_{k+1} \cdots \lor D_n \big)}_{C_m} \]
where each $D_i$ represents a single positive or negative constraint,  $D(\textbf{a}_\textbf{i}, \textbf{y})$ or $\neg D(\textbf{a}_\textbf{i}, \textbf{y})$, restricting whether key phrase $\textbf{a}_\textbf{i}$ should be strictly included or omitted in \textbf{y}, respectively. \citeauthor{lu-etal-2021-neurologic} refer to each individual constraint $D_i$ as a \emph{literal}, and the disjunction of literals as a \emph{clause}, denoted as $C_j$. \methodshort seeks optimal sequences in which all clauses are satisfied.
 By introducing penalties \cite{Fiacco1976SensitivityAF}, \citeauthor{lu-etal-2021-neurologic} approximate the constrained optimization problem with an unconstrained problem.
\vspace*{-3mm}
\begin{align*}
    \hat{\textbf{y}} = &\arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x}) - \lambda' \sum_{i=1}^{L} (1-C_i)
 \end{align*}
 While exhaustive search is intractable, \citeauthor{lu-etal-2021-neurologic} uses a beam-based search to find approximately-optimal solutions for this objective. 
At each time step, \methodshort chooses which candidates to expand next by 3 steps: \emph{pruning}, \emph{grouping}, and \emph{selecting} 

\textbf{Pruning step}: \methodshort first discards any $h$ with irreversible unsatisfied clauses, and then drop any candidates not in the top-$\alpha$ in terms of likelihood $P_\theta(\textbf{y}_t|\textbf{y}_{<t})$, and not in the top-$\beta$ in terms of number of satisfied clauses $\sum_{i=1}^{L} C_i$. 

\textbf{Grouping step}: Next, \methodshort selects the beam from the pruned candidates. \citeauthor{lu-etal-2021-neurologic} consider diverse partial solutions to avoid satisfying constraints in a greedy manner. \methodshort groups candidates based on the set of irreversible satisfied clauses and select (in the next step) the best ones from each group to fill the beam. 

\textbf{Selecting step}: To select best ones from each group, \methodshort first ranks candidates within a group by score function:
\vspace*{-3mm}
\begin{align*}
\textbf{s} = &\> P_\theta(\textbf{y}_t|\textbf{x}, \textbf{y}_{<t}) + \lambda_1 \cdot \max_{\substack{D(\textbf{a}_\textbf{i}, \textbf{y}) \\ \in \> \textnormal{state S1}}} \frac{|\hat{\textbf{a}}_\textbf{i}| }{|\textbf{a}_\textbf{i}|}
 \end{align*}
The second term denotes the partial reward to candidates moving towards satisfying a positive literal in an unsatisfied clause. \methodshort then proceeds in rounds of filling the beam, visiting each group and taking the best scoring ones in rotation, until reach $k$ candidates. 

\subsection{Our Approach: \Aneurologic}
\method improves upon the scoring function. The original scoring function gives reward to candidates in the middle of generating a new positive constraint only, and ranks the rest of candidates by purely likelihood. However, even if a candidate doesn't in the process of generating a new constraint yet, we should consider the effect of its current generation to satisfying another unsatisfied constraint in the near future. In other words, we should encourage candidates which are more context relevant to an unsatisfied constraint so that this constraint can be inserted in a more fluent and coherent way in the future. Hence, we propose scoring function as 
\begin{align*}
\textbf{s} = &\> P_\theta(\textbf{y}_t|\textbf{x}, \textbf{y}_{<t}) + \lambda_1 \cdot \max_{\substack{D(\textbf{a}_\textbf{i}, \textbf{y}_{1:t}) \\ \in \> \textnormal{state S1}}} \frac{|\hat{\textbf{a}}_\textbf{i}| }{|\textbf{a}_\textbf{i}|} + \lambda_2 \max_{\substack{D(\textbf{a}_\textbf{i}, \textbf{y}_{1:t}) \\ \in \> \textnormal{state S1}}} \tilde{P}_\theta \Big(D(\textbf{a}_\textbf{i}, \textbf{y}_{t+1:t+k})\myeq\textnormal{True}\big|\textbf{x}, \textbf{y}_{1:t}\Big)
 \end{align*}
where $D(\textbf{a}_\textbf{i}, \textbf{y}_{t+1:t+k})$ is a boolean function indicating whether key phrase $\textbf{a}_\textbf{i}$ appears in generation $\textbf{y}_{t+1:t+k}$, and $P_\theta(D(\textbf{a}_\textbf{i}, \textbf{y}_{t+1:t+k})\myeq\textnormal{True}|\textbf{x}, \textbf{y}_{1:t})$ denotes the probability that key phrase $\textbf{a}_\textbf{i}$ gets generated in next $k$ steps conditioned on current candidates. Overall, the second term gets reward to candidates which are more likely to satisfy \emph{one more} literal constraint in the near future.  

We first factorize the probability in the second term for a certain literal $\textbf{a}_\textbf{i}$ over time step
\[\tilde{P}_\theta\Big(D(\textbf{a}_\textbf{i}, \textbf{y}_{t+1:t+k})\myeq\textnormal{True}\big|\textbf{x}, \textbf{y}_{1:t}\Big)= \max_{i\in [1,k]}\tilde{P}_\theta\Big(\textbf{y}_{t+i:t+i+|\textbf{a}_\textbf{i}|} \myeq \textbf{a}_\textbf{i}\big|\textbf{x}, \textbf{y}_{1:t+i-1}\Big)\]
Then, we leverage future state obtained by \method to estimate the the probability that a new literal constraint $\textbf{a}_\textbf{i}$ will appear in generation starting at $\textbf{y}_{t+i}$. 
\vspace*{-3mm}
\[\tilde{P}_\theta\Big(\textbf{y}_{t+i:t+i+|\textbf{a}_\textbf{i}|} \myeq \textbf{a}_\textbf{i}\big|\textbf{x}, \textbf{y}_{1:t+i-1} \Big)
= \prod_{j=0}^{|\textbf{a}_\textbf{i}|} \tilde{P}_\theta(\textbf{y}_{t+i+j}\myeq \textbf{a}_\textbf{i}^j|\textbf{x}, \textbf{y}_{1:t+i-1}, \textbf{y}_{t+i-1:t+i+j-1} \myeq \textbf{a}_\textbf{i}^{<j})\]
where $\textbf{a}_\textbf{i}^{j}$ and $\textbf{a}_\textbf{i}^{<j}$ denotes the $j$th token and the first $j \mkern0.1mu{-}\mkern0.1mu 1$ tokens of the key phrase $\textbf{a}_\textbf{i}$ separately. The word representation of $\textbf{y}_{1:t+i-1}$ is obtained by concatenating the word embedding of $\textbf{y}_{1:t}$ and the fuzzy word embedding of $\textbf{y}_{t+1:t+i-1}$, and word representation of $\textbf{y}_{1:t+i-1}$ is the word embedding of $\textbf{a}_\textbf{i}^{<j}$.

==> section/2_method_new_archive.tex <==

\section{A$^*$ NeuroLogic Decoding with Lookahead}
\liwei{need a different (more concrete) section title, e.g., A-star neurologic decoding with lookahead heuristic}

\liwei{Could we start the method section with a high level description of A-star decoding before diving into the technical details and equations?}\sean{yes}

We introduce the decoding problem, describe our lookahead heuristics, then describe how we adopt them for lexically-constrained generation.

\paragraph{Background: Decoding.}
Sequence-to-sequence generation is the task of generating an output sequence $\yb$ given an input sequence $\xb$. 
We consider standard autoregressive models, 
$p_\theta(\yb|\xb) = \prod_{t=1}^{|\yb|} p_\theta (\yb_t| \yb_{<t},\xb)$, and
omit $\xb$ to reduce clutter.
Decoding consists of solving,
\begin{align}
\label{eqn:decode}
\yb_* = \argmax_{\yb\in \mathcal{Y}} V(\yb),
\end{align}
where $V(\yb)$ is a scoring function.
In our setting, $V(\yb)$ takes the form $\log p_\theta(\yb)+H(\yb)$, where $H(\yb)$ is either zero or enforces constraints on $\yb$.
%

Our method takes the perspective of decoding as discrete search, in which states are partial prefixes, $\yb_{<t}$, actions are tokens, $y_t\in \mathcal{V}$, and transitions add a token to a prefix, $\yb_{<t}\circ y_t$.
Each step of decoding consists of expanding a set of candidate next-states, evaluating each candidate using an approximation to $V(\yb)$, and selecting the $k$ best candidates:
\begin{align}
\label{eqn:update}
    \nonumber Y_{t}' &= \{\yb_{<t}\circ y_t\ |\ \yb_{<t}\in Y_{t-1}, y_t\in \mathcal{V}\},\\
    Y_{t}  &=\argtopk_{(\yb_{<t},y_t)\in Y_{t}'}\ \left\{\hat V(\yb_{< t}, y_t)\right\},
\end{align}
where $Y_0 = \{\langle bos \rangle\}$.
Common decoding algorithms such as beam search approximate the objective $V$ without considering future tokens, e.g. $\hat V(\yb_{<t}, y_t)=\log p_\theta(\yb_{\leq t})$.

\paragraph{Lookahead heuristics.}
We want to select next-tokens $y_t$ that keep the expanded prefixes on optimal trajectories, replacing \autoref{eqn:update} with:
\begin{align}
\label{eqn:update2}
    Y_t=\argtopk_{(\yb_{<t},y_t)\in Y_{t}'}\ \left\{ Q(\yb_{<t},y_t) \right\},
\end{align}
where, 
\begin{align}
\label{eqn:qfunc}
Q(\yb_{<t},y_t)=\max_{\yb_{>t}} V(\yb_{<t},y_t,\yb_{>t}).
\end{align}
However, computing \autoref{eqn:qfunc} presents two difficulties: (1) the space of future trajectories $\yb_{>t}$ is prohibitively large, and (2) the true objective $V(\yb)$ may be unknown or difficult to compute.

To address the first difficulty, we approximate $Q$ using a \textit{lookahead}:
\begin{align*}
    \hat{Q}_{k}(\mathbf{y}_{<t},y)=\max_{\yb_{t+1:t+k}\in S_k(\yb_{\leq t})} \hat V(\yb_{<t},y_t,\yb_{t+1:t+k}),
\end{align*}
where each element $\yb_{t+1:t+k}$ of  $S_k(\yb_{\leq t})$ is a length-$k$ continuation of $\yb_{\leq t}$.
%

To address the second difficulty, we approximate the decoding objective using a \textit{heuristic} computed on the expanded prefixes obtained with lookahead,
\begin{align*}
    \hat V(\yb_{\leq t+k})=\log p_\theta(\yb_{\leq t})+h(\yb_{\leq t+k}).
\end{align*}
Beam search corresponds to setting $k$ and $h$ to 0.

\paragraph{Generating lookaheads.}
We compare 3 methods for generating the lookaheads $S_k(\yb_{\leq t})$.
The \textbf{greedy} lookahead produces a single sequence, $S_k=\{\yb_{t+1:t+k}\}$, starting from $\yb_{\leq t}$ and selecting each token according to
$y_{t'} =\argmax_{y\in \mathcal{V}} p_\theta(y|\mathbf{y}_{< t'})$.
The greedy lookahead is efficient, but only explores a single trajectory.

The \textbf{beam} lookahead trades off efficiency for exploration, returning a set $S_k$ containing the top-$B$ candidates obtained by running beam search for $k$ steps starting from $\yb_{<t}$ with width $B$.

Finally, the \textbf{sampling} lookahead explores beyond the highly-probable beam search continuations, generating  each $\yb_{t+1:t+k}\in S_k$ using,
\begin{align*}
    y_{t'} \sim p_\theta(y|\mathbf{y}_{< t'}),
\end{align*}
for $t'$ from $t$+1 to $t$+k.

\paragraph{Connection with A$^{*}$ search.}
Our method is an instance of A$^{*}$ search~\citep{hart1968}, 
a best-first search algorithm that finds low-cost paths by selecting actions which minimize,
$$f(a)=g(a)+h(a),$$ where $g(a)$ is the cost-so-far and $h(a)$ is a heuristic estimate of future cost.
In our case, $g(a)$ is $\log p_{\theta}(\yb_{\leq t})$, and $h(a)$ is our lookahead heuristic $h(\yb_{\leq t+k})$.
Given this connection, we refer to our method \textit{A$^*$-decoding with lookahead heuristics}, or \textit{lookahead decoding} for short.
% \textit{A* decoding with lookahead}, or \textit{lookahead decoding}.

% \if 0
\paragraph{Does lookahead improve search?}
As the lookahead length $k\rightarrow \infty$ and number of lookaheads $|S_k|\rightarrow \infty$, it is easy to see that lookahead decoding exactly solves \autoref{eqn:qfunc}. 

The correspondence with A$^*$ search implies that for practical choices of $k$ and $|S_k|$, if the heuristic $h(\yb_{\leq t+k})$ is \textit{admissible} -- i.e. $h(\yb_{\leq t+k})\geq H(\yb_*)$ for all $\yb_{\leq t+k}$ -- and the beam width is sufficiently large, lookahead decoding will return an optimal sequence.
However, these guarantees do not necessarily apply for practical beam sizes, so we 
% However, using an admissible heuristic is a sufficient, but not necessary, condition.
evaluate our lookahead heuristics empirically, and save further theoretical analysis as future work.
% \fi

Next, we move to our proposed lookahead heuristics, starting with the unconstrained setting.


==> section/old_text.tex <==
%%%%%%%%% copying old text here before I edit them so that we don't lose them 


\begin{abstract}


Despite the promising progress in neural language modeling (LMs), it remains an open question what the best decoding heuristic is for text generation from a language model. The dominant approaches involve sampling from or maximizing sequence likelihood, such as beam search, top-k or nucleus sampling.  
However, many neural text degeneration cases are reported with likelihood-based
decoding methods: output text that is repetitive, incoherent, or generic \citep{holtzman2020curious}.

We propose \textsc{A$^\textbf{*}$ Heuristic}, an alternative decoding heuristic that enables left-to-right language models to leverage estimated future state to guide current generation.
Empirical results on 5 generation benchmarks show that \method decodes higher quality text out of neural language models on top of both beam-based and sampling-based decoding methods.

Moreover, we generalize \method to constrained generation, where the objective is to maximize both sequences likelihood and constraint satisfaction. Empirical results on C{\small OMMON}G{\small EN} \liwei{Why do we only mention commongen in the abstract, as we have six tasks? Or maybe we can say a wide range of NLG tasks? Or can we specifically mention six tasks in the abstract, to show our diverse/wide coverage of different tasks?} demonstrate noticeable performance boosts brought by \method over \neurologic, a start-of-art constrained generation method. Furthermore, \method enables direct application of \neurologic with  off-the-shell pre-trained LMs to non-sequential generation tasks such as template filling and storyline-guided storytelling.
\jungo{the preceding sent is a bit confusing; isn't \neurologic directly applicable without A star as well?}
Our results suggest the promise of proposed \method and the limit of existing decoding methods, in both unconstrained and constrained settings.


\lianhui{ Nice abstract! I re-ordered and shortened the current version a bit and made a rough draft. Feel free to edit if something is not accurate. \\
Neural text generation with likelihood-based decoding strategies, such as greedy, beam search, top-k sampling, has achieved impressive results of generating human-like fluent and logical text. However, the likelihood-based decoding is also shown to suffer from text degeneration (Holtzman et al., 2020a), i.e., outputing text that is repetitive, incoherent, or overly generic. \liwei{maybe re-order the first two sentences to pinpoint the problem of existing decoding methods first, then briefly mention they are impressive. E.g., existing decoding methods are known to have problems, such as..., despite they show impressive results} We hypothesize that directly sampling from or maximizing sequence likelihood at each local step from left to right, as in the previous methods, is an insufficient decoding heuristic. \liwei{The previous sentence seems to be more important than first two sentences, as the main shortcoming of existing methods is they only sample from left-to-right. We could potentially start the abstract with this sentence, to straightforwardly point out this main shortcoming of existing methods, which directly motivates A-star decoding.} We propose A* HEURISTIC, a new alternative \liwei{new and alternative are a bit redundant} decoding heuristic that improves generation quality \liwei{improves generation quality is a bit vague} and avoids degeneration by leveraging estimated future state to guide current generation. We develop simple lookahead strategies for effective future state estimation. Moreover, \liwei{may not need moreover} A* HEURISTIC enables off-the-shell left-to-right pre-trained LMs to perform constrained non-monotonic text generation, such as text infilling, lexical constrained decoding.  Empirical results \liwei{across X tasks} demonstrate improved generation quality brought by A* HEURISTIC on-top-of existing likelihood-based decoding methods in both unconstrained and constrained settings. }

\liwei{maybe we should mention how many SOTA A-star achieves}

\begin{comment}
Neural text generation is important for a wide range of downstream natural language applications. However, the standard approach -- using a finetuned language models (LMs) \citep{Vaswani2017AttentionIA, radford2019language} with  maximization- or sampling-based decoding strategies – is known to exhibit \textit{de}generation \citep{welleck2020neural}. \liwei{Can we briefly explain what degeneration means in the intro, in case some readers don't know?} \daniel{+1; and clarify what is it about A*/lookahead that addresses "degeneration"} Despite being pre-trained on large amounts of data, text generated by neural models is observed to be repetitive, generic, incoherent, and self-contradictory \citep{holtzman2020curious}.
\daniel{I am not sure if this is the right way to motivate the world. 
I think you need to argue the current decoding algorithms are not informed of the future expectations/constraints over the course of generation. Which would motivate the use of "lookahead". 
}

Many explanations have been proposed for neural text degeneration, including inappropriate training objectives \citep{welleck2020neural} and decoding discrepancies relative to human language \citep{holtzman-etal-2018-learning, holtzman2020curious}.  While the aforementioned may be factors for neural degeneration, we hypothesize that 
directly sampling from or maximizing sequence likelihood is an insufficient decoding heuristic \liwei{can we be more specific about our hypothesis? E.g., generating logical texts or constructing fluent texts usually require project into the future/taking future content into account/plan ahead to have a holistic view}, and thus associated with neural text degeneration. We proposed \method, an alternative decoding heuristic that leverages estimated future state to guide current generation. Empirical results demonstrate improved generation quality brought by \method on-top-of existing likelihood-based decoding methods in both unconstrained and constrained settings.
\end{comment}



Recent work  on text generation with lexical constraints has shown  promising results. 
However, because of unidirectional nature of these algorithms (often left to right) they suffer from the lack of foresight about future constraints. 
% Standard sequential  generation from language models assume a pre-specified generation order (typically from left to right) which makes them blind about their future generations and the necessary constraints. 
% \ximing{I think what we proposed is a look-ahead heuristics, which can be used in conventional beam search, sampling, or \neurologicshort. When the look-ahead heuristics is used in \neurologicshort, we call the entire algorithm \methodnospace esq. I'm not sure saying "we propose \methodnospace" is clear enough. }
In this work, we build upon  \neurologicshort{}, a recently proposed constraint decoding algorithm~\cite{lu-etal-2021-neurologic} by augmenting it with \emph{look-ahead heuristics} (estimated future gains from each generation) to guide its generation towards those that satisfy logical constraint while maintaining a  fluent and coherent language. 
% leveraging estimated future state to guide current generation is most helpful
% Such guided generation, we show, can augment (and improve) existing generation techniques, such as greedy decoding or beam search. 
% In particular, our proposal combines look-ahead heuristics with \neurologicshort{} decoding~\cite{lu-etal-2021-neurologic}, a prior constrained decoding algorithm for predicate constraints, which  enables non-monotonic text generation for a variety of long-distance constraints, such as text infilling, lexical constrained decoding. 
We evaluate the resulting algorithm, \method on 5 generation benchmarks and where  it consistently leads to higher quality text out of neural language models -- supervised or not. 
These gains are particularly notable in setups with limited task supervision  where informed search about ensuing constraints is necessary.  
Our results suggest the promise of the proposed \method  decoding algorithms for a variety of tasks and setups via off-the-shell left-to-right pre-trained LMs.

\peter{New version with A*esque below}


